Language-Parametric Reference Synthesis (Extended)

Modern Integrated Development Environments (IDEs) offer automated refactorings to aid programmers in developing and maintaining software. However, implementing sound automated refactorings is challenging, as refactorings may inadvertently introduce name-binding errors or cause references to resolve to incorrect declarations. To address these issues, previous work by Sch\"afer et al. proposed replacing concrete references with locked references to separate binding preservation from transformation. Locked references vacuously resolve to a specific declaration, and after transformation must be replaced with concrete references that also resolve to that declaration. Synthesizing these references requires a faithful inverse of the name lookup functions of the underlying language. Manually implementing such inverse lookup functions is challenging due to the complex name-binding features in modern programming languages. Instead, we propose to automatically derive this function from type system specifications written in the Statix meta-DSL. To guide the synthesis of qualified references we use scope graphs, which represent the binding structure of a program, to infer their names and discover their syntactic structure. We evaluate our approach by synthesizing concrete references for locked references in 2528 Java, 196 ChocoPy, and 49 Featherweight Generic Java test programs. Our approach yields a principled language-parametric method for synthesizing references.

==> Makefile <==
# Directory with the source files
SRCDIR      = src
# Directory with the library files
LIBDIR      = lib
# Directory where the build files are located
BUILDDIR    = build
# Directory where the PDF is copied
DOCDIR      = .
DOCNAME     = main
# The path to the main .tex file
MAINTEX     = main.tex
# Directory for the PDF snapshots
SNAPDIR     = snapshots
# Prefix for PDF snapshots
SNAPNAME    = reference-synthesis
# Directory for the source archives
ARCHIVEDIR  = archive
# Name for source archives
ARCHIVENAME = reference-synthesis
# Researchr bibliography file
SRCBIB      = bibliography.bib
# Source files
SRCFILES    = $(MAINTEX) $(SRCBIB) \
	$(wildcard $(SRCDIR)/*.tex) \
	$(wildcard $(SRCDIR)/**/*.tex) \
	$(wildcard $(SRCDIR)/*.bib) \
	$(wildcard $(SRCDIR)/*.png) \
	$(wildcard $(SRCDIR)/*.cls) \
	$(wildcard $(SRCDIR)/*.bst) \
	$(wildcard $(SRCDIR)/*.pdf) \
	$(wildcard $(LIBDIR)/*) \
	latexmkrc
# Researchr bibliography name
RESEARCHR   = reference-retention

LATEXMK     = latexmk
LIVE        = -pvc -view=none -halt-on-error
DOCUMENT    = $(DOCDIR)/$(DOCNAME).pdf

# Build the PDF
all: $(DOCUMENT)

# Build a PDF
%.pdf: %.tex $(SRCFILES)
	@echo "Warning: Underfull and overfull box warnings are suppressed!"
	$(LATEXMK) "$<" -jobname=${*F}
	@echo "Done building $@"


# Download the latest bibliography from Researchr and fix it
bib: clean-bib $(SRCBIB)
$(SRCBIB):
	curl -s "https://researchr.org/downloadbibtex/bibliography/$(RESEARCHR)" -o $@
	sed -i '' '1 s/^/% /' $@
	sed -i '' 's/doi = {http.*\/\(10\..*\)}/doi = {\1}/' $@
	sed -i '' '/doi = {http.*}/d' $@
	sed -i '' 's/\&uuml;/ü/' $@
	@echo "Updated $@ from https://researchr.org/downloadbibtex/bibliography/$(RESEARCHR)"

# Remove the bibliography
clean-bib:
	-@rm -f $(SRCBIB)

# Removes PDF build files
clean:
	-@$(LATEXMK) -C $(DOCUMENT)

# Removes all build files
clean-all: clean clean-bib
	-@rm -r $(BUILDDIR)/

# Watch for changes and rebuild
watch:
	$(LATEXMK) $(LIVE) $(MAINTEX) -jobname=$(DOCNAME)

# Copy the latest built PDF to the snapshots directory
snapshot: $(DOCUMENT)
	mkdir -p $(SNAPDIR)
	cp "$<" $(SNAPDIR)/$(shell date +"%Y%m%dT%H%M%S")-$(SNAPNAME).pdf

# Create an archive with the source files
archive: $(DOCUMENT)
	$(eval ARCHIVEFILE := $(abspath $(ARCHIVEDIR)/$(shell date '+%Y%m%d%H%M')-$(ARCHIVENAME).zip))
	mkdir -p $(ARCHIVEDIR)
	-@rm $(ARCHIVEFILE) 2> /dev/null
	cd $(SRCDIR)     && zip        $(ARCHIVEFILE) $(shell cd $(SRCDIR)     && find . -type f \( -name '*.tex' -o -name '*.bib' -o -name '*.png' -o -name '*.cls' -o -name '*.bst' -o -name '*.pdf' \) -not -path './dataviz/*')
	cd $(LIBDIR)     && zip --grow $(ARCHIVEFILE) $(shell cd $(LIBDIR)     && find . -type f)
	cd $(BUILDDIR)   && zip --grow $(ARCHIVEFILE) $(shell cd $(BUILDDIR)   && find . -type f -name '*.bbl')
	cd .             && zip --grow $(ARCHIVEFILE) $(shell cd .             && find . -type f -maxdepth 1 -name '*.tex' -o -name 'README.md' -o -name 'Makefile' -o -name 'latexmkrc')

.PHONY: all bib clean-bib clean clean-all watch snapshot archive check
.SILENT:
.SUFFIXES: .pdf
.PRECIOUS: $(DOCUMENT)


==> fig/0600-chocopy-summary-table.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% This file is generated using `python3 dataviz.py` in `evaluation/dataviz/`
% Based on this result set: 20240929T173103
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{tabular}{|l|r|r|r|r|r|r|r|}
  \hline
  ChocoPy & Min & $P_{5\%}$ & $P_{25\%}$ & Median & $P_{75\%}$ & $P_{95\%}$ & Max \\
  \hline
  \hline
  Character count & 22 & 33 & 79 & 160 & 324 & 991 & 3198 \\
  Line count & 4 & 5 & 8 & 13 & 20 & 60 & 189 \\
  Token count & 16 & 21 & 38 & 78 & 134 & 432 & 1753 \\
  AST count & 15 & 20 & 33 & 66 & 112 & 363 & 1390 \\
  Hole count & 1 & 1 & 3 & 6 & 12 & 46 & 161 \\
  \hline
  Initial analysis time (ms) & 5 & 7 & 13 & 23 & 41 & 105 & 656 \\
  Average synthesis time per hole (ms) & 5 & 11 & 29 & 69 & 387 & 6671 & 7505 \\
  Synthesis time (ms) & 11 & 33 & 104 & 286 & 8759 & 60192 & 60474 \\
  Total time (ms) & 26 & 52 & 131 & 330 & 8806 & 60295 & 61512 \\
  \hline
\end{tabular}

==> fig/0600-example-evaluation-test-file.tex <==
%% moveClass/conflictingNames_before
\begin{lstlisting}[
  language=Java,
]
test;
[`\posidc{p2}{1}`] {
  [Test]
    package p2;
    public class `\posidc{Test}{2}` {
      public static void `\posidc{f}{3}`() {}
    }
  [First]
    package p2;
    public class `\posidc{First}{4}` {}
}
[p1] {
  [Second]
    package p1;

    import `\rholec[6]{\posidc{p2}{1}}`.*;

    class `\posidc{Second}{5}` {
      {
        new `\rholec[9]{\posidc{First}{6}}`();
        `\rholec[6]{\posidc{f}{3}}`();
      }
    }
  [First]
    package p1;
    public class `\posidc{First}{6}`
      extends `\rholec[9]{\posidc{First}{4}}` {}
}
\end{lstlisting}%

==> fig/0600-fgj-summary-table.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% This file is generated using `python3 dataviz.py` in `evaluation/dataviz/`
% Based on this result set: 20240929T173103
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{tabular}{|l|r|r|r|r|r|r|r|}
  \hline
  FGJ & Min & $P_{5\%}$ & $P_{25\%}$ & Median & $P_{75\%}$ & $P_{95\%}$ & Max \\
  \hline
  \hline
  Character count & 78 & 101 & 152 & 241 & 348 & 493 & 926 \\
  Line count & 6 & 7 & 10 & 14 & 19 & 27 & 45 \\
  Token count & 52 & 63 & 87 & 136 & 215 & 252 & 426 \\
  AST count & 20 & 28 & 40 & 62 & 88 & 119 & 203 \\
  Hole count & 1 & 1 & 3 & 5 & 10 & 18 & 44 \\
  \hline
  Initial analysis time (ms) & 32 & 36 & 52 & 62 & 77 & 113 & 179 \\
  Average synthesis time per hole (ms) & 15 & 25 & 48 & 106 & 1363 & 5004 & 6002 \\
  Synthesis time (ms) & 42 & 65 & 125 & 292 & 14313 & 60053 & 60132 \\
  Total time (ms) & 112 & 126 & 206 & 415 & 14375 & 60140 & 60244 \\
  \hline
\end{tabular}

==> fig/0600-java-summary-table.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% This file is generated using `python3 dataviz.py` in `evaluation/dataviz/`
% Based on this result set: 20240929T173103
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{tabular}{|l|r|r|r|r|r|r|r|}
  \hline
  Java & Min & $P_{5\%}$ & $P_{25\%}$ & Median & $P_{75\%}$ & $P_{95\%}$ & Max \\
  \hline
  \hline
  Character count & 64 & 120 & 192 & 276 & 391 & 735 & 2374 \\
  Line count & 6 & 10 & 14 & 17 & 22 & 31 & 75 \\
  Token count & 37 & 66 & 93 & 120 & 158 & 242 & 541 \\
  AST count & 23 & 47 & 69 & 91 & 121 & 193 & 475 \\
  Hole count & 1 & 1 & 2 & 3 & 6 & 13 & 43 \\
  \hline
  Initial analysis time (ms) & 11 & 15 & 23 & 35 & 55 & 103 & 449 \\
  Average synthesis time per hole (ms) & 3 & 7 & 13 & 26 & 107 & 4090 & 20016 \\
  Synthesis time (ms) & 4 & 10 & 28 & 86 & 608 & 60014 & 60813 \\
  Total time (ms) & 20 & 32 & 61 & 140 & 682 & 60077 & 60836 \\
  \hline
\end{tabular}
